Peak-Aware Online Economic Dispatching for Microgrids

By employing local renewable energy sources and power generation units while connected to the central grid, microgrid can usher in great benefits in terms of cost efficiency, power reliability, and environmental awareness. Economic dispatching is a central problem in microgrid operation, which aims at effectively scheduling various energy sources to minimize the operating cost while satisfying the electricity demand. Designing intelligent economic dispatching strategies for microgrids, however, is drastically different from that for conventional central grids, due to two unique challenges. First, the erratic renewable energy emphasizes the need for online algorithms. Second, the widely-adopted peak-based pricing scheme brings out the need for new peak-aware strategy design. In this paper, we tackle these critical challenges and devise peak-aware online economic dispatching algorithms. For microgrids with fast-responding generators, we prove that our deterministic and randomized algorithms achieve the best possible competitive ratios $2-\beta$ and $e/(e-1+\beta)$, respectively, where $\beta\in[0,1]$ is the ratio between the minimum grid spot price and the local-generation price. Our results characterize the fundamental \emph{price of uncertainty} of the problem. For microgrids with slow-responding generators, we first show that a large competitive ratio is inevitable. Then we leverage limited prediction of electricity demand and renewable generation to improve the competitiveness of the algorithms. By extensive empirical evaluations using real-world traces, we show that our online algorithms achieve near offline-optimal performance. In a representative scenario, our algorithm achieves $17.5\%$ and $9.24\%$ cost reduction as compared to the case without local generation units and the case using peak-oblivious algorithms, respectively.

==> App.tex <==
%\section{Appendix}\label{sec:app}
\appendix
\section{Proof of Proposition 1}\label{proof:ratio}

\begin{proof}
We denote the number of time slots with demand $1$ by $T$, and the number of time slot using the local generator before turning to the grid by $T^s$. Two inequalities $z p_m \leq T(p_g-p_e^{\min})$, $s p_m \leq T(p_g-p_e^{\min})$ are used in the following.

$\vartriangleright$ \textbf{Case 1:} ${z \leq 1}$. The optimal offline solution is always using the local generator and the cost is $\text{Cost}_{\text{off}} = Tp_g$.

\hspace{0.5cm}$\vartriangleright$ \textbf{Case 1.1:} $s> z$. In this case, the online algorithm will not turn to the grid before the input ends. Therefore, the online cost is exactly  the same as the   offline cost, thereby the ratio is $1$.

\hspace{0.5cm}$\vartriangleright$ \textbf{Case 1.2:} $s \leq z$. It turns out that there is a critical time slot $T^s$ that for all  $1 \leq t\leq T^s$, the online algorithm uses the local generator and for  time slots $T^s < t \leq  T$, it turns to the grid, thereby we have ${\text{Cost}_{\text{on}} = T^sp_g+\sum_{t = T^s+1}^{t=T}p_e(t)+p_m}$.
%However, the offline algorithm satisfies the total demand for the whole time horizon from the local generator (${\text{Cost}_{\text{off}} = Tp_g}$).
Hence, we get the following ratio:
\begin{align*}
R(s,z) &= \frac{T^sp_g+\sum_{t = T^s+1}^{t=T}p_e(t)+p_m}{Tp_g}\\
%&=\frac{Tp_g-(T-T^s)p_g+\sum_{t = T^s+1}^{t=T}p_e(t)+p_m}{Tp_g}\\
&=1+\frac{\sum_{t=1}^{T^s}(p_g-p_e(t))-\sum_{t=1}^{t=T}(p_g-p_e(t))+p_m}{Tp_g}\\
%&\leq1+\frac{s p_m-z p_m+p_m}{Tp_g}\\
& \leq 1+(1-z+s)\frac{p_m}{T p_g}\\
&\leq 1+\frac{1-z+s}{z}\frac{p_g-p_e^{\min}}{p_g}\\
&=1+\frac{1-z+s}{z}(1-\beta)
\end{align*}
%The last inequality is due to the fact that ${z p_m = \sum(p_g-p_e(t))\leq T(p_g-p_e^{\min})}$.

$\vartriangleright$ \textbf{Case 2:} $z > 1$. The optimal offline solution is always acquiring the electricity from the grid and the cost is ${\text{Cost}_{\text{off}}=\sum_{t=1}^{T} p_e(t)+p_m}$.

\hspace{0.5cm}$\vartriangleright$ \textbf{Case 2.1:} $s> z$, In this case, the online algorithm always uses the local generator and thus the online cost is ${\text{Cost}_{\text{on}} = Tp_g}$. Hence, the ratio is as follows:
\begin{align*}
R(s,z) &= \frac{Tp_g}{\sum_{t=1}^{T} p_e(t)+p_m}\\
& = 1+\frac{\sum_{t=1}^{T}(p_g-p_e(t))-p_m}{\sum_{t=1}^{T} p_e(t)+p_m}\\
%& \leq 1+\frac{(z-1)p_m}{Tp_e^{\min}+p_m}\\
& \leq 1+\frac{(z-1)}{p_e^{\min}\frac{T}{{p_m}}+1}\\
& \leq 1+\frac{(z-1)}{p_e^{\min}\frac{z}{p_g-p_e^{\min}}+1}\\
%& = 1+\frac{(z-1)(p_g-p_e^{\min})}{(z-1)p_e^{\min}+p_g}\\
& = 1+\frac{(z-1)(1-\beta)}{(z-1)\beta+1}
\end{align*}
%where the last inequality is true since  $z p_m \leq T(p_g-p_e^{\min})$.

\hspace{0.5cm}$\vartriangleright$ \textbf{Case 2.2:} $s\leq z$. Like case 2.1 here we have  $T\geq T^s$. Therefore, the online algorithm  uses the local generator for the first $T^s$ time slots and turns to the grid afterwards. In this case, the online cost is ${\text{Cost}_{\text{on}} = T^sp_g+\sum_{t = T^s+1}^{t=T}p_e(t)+p_m}$, and the ratio is
\begin{align*}
R(z,s) &= \frac{T^sp_g+\sum_{t = T^s+1}^{t=T}p_e(t)+p_m}{\sum_{t=1}^{T} p_e(t)+p_m}\\
& =1+ \frac{\sum_{t=1}^{T^s}(p_g-p_e(t))}{\sum_{t=1}^{T} p_e(t)+p_m}\\
%&\leq 1+\frac{sp_m}{Tp_e^{\min}+p_m}\\%, \text{by }\sum_{t=1}^{T^s}(p_g-p_e(t)) \leq sp_m\\
%& = 1+\frac{s}{p_e^{\min}\frac{T}{p_m}+1}\\
& \leq 1+\frac{s}{p_e^{\min}\frac{z}{p_g-p_e^{\min}}+1}\\
%& = 1+\frac{s(p_g-p_e^{\min})}{(z-1)p_e^{\min}+p_g}\\
& = 1+\frac{s(1-\beta)}{(z-1)\beta+1}
\end{align*}

The proof is completed.
\end{proof}
\iffalse
\subsection{Proof of Lemma \ref{lemma:ramping_feasibility}}\label{proof:ramping_feasibility}

\begin{proof}
By the obtainment of $\tilde{u}(t+1)$, we can have $\tilde{u}(t+1)\geq \tilde{u}(t)-R$, i.e
$$\tilde{u}(t)-\tilde{u}(t+1)\leq R$$

Next, we prove $\tilde{u}(t+1)-\tilde{u}(t)\leq R$ for two cases.

Firstly, if $\tilde{u}(t+1) = (\tilde{u}(t)-R)^+$, the conclusion holds obviously.

Secondly, if for some $i^*\in[0,w-1]$ such that $\tilde{u}(t+1) = u(t+1+i^*)-i^*R$, we can have


\begin{align*}
\tilde{u}(t+1) &=\max\{0, u(t+1+i)-iR|i\in[0,\omega-1]\}\\
&=\max\{0,u(t+1+i)-(i+1)R+R|i\in[0,\omega-1]\} \\
&=\max\{0,u(t+j)-jR|j\in [1,\omega]\}+R\}\\
&=\max\{0,u(t+j)-jR|j\in [1,\omega-1]\}+R\}
\end{align*}

The last step is due to the fact that $u(t+w)\leq C\leq wR$. and since $\tilde{u}(t) =\max\{0,\tilde{u}(t-1)-R, \max\{u(t+j)-jR|i\in [0,w-1]\}\}$, we can have $\tilde{u}(t)\geq \max\{0,u(t+j)-jR|j\in[0,\omega-1]\}\geq \{0,u(t+j)-jR|j\in[1,\omega-1]\}$.

Then it's easy to see that $\tilde{u}(t+1) \leq \tilde{u}(t)+R$, i.e
$$\tilde{u}(t+1)-\tilde{u}(t)\leq R$$
which means the ramping up constraint is satisfied and the proof is completed.
\end{proof}

\subsection{Proof of Theorem \ref{theorem:CR_ramp}}\label{proof_ramping_CR}
\begin{proof}

According to the algorithm we can easily get
\begin{lemma}\label{lemma:ramping_cost_grid}
For $\tilde{u}(t)$,$\tilde{v}(t)$ obtain by \algc, we can have
$\tilde{v}(t)\leq v(t)$, and thus $\max_t\tilde{v}(t)\leq \max_t v(t)$
\end{lemma}

We denote the online cost of Algorithm~\ref{Alg:ramping} as $\tilde{C}_{\text{on}}$ and the optimal offline cost of the same problem as $\tilde{C}_{\textrm{off}}$. For the problem without ramping constraints, we denote the online cost of Algorithm~\ref{alg:online} as $C_{\textrm{on}}$ and the optimal offline cost of the same problem as $C_{off}$. We can directly have $\tilde{C}_{\textrm{off}}\geq C_{\textrm{off}}$. Then
\begin{align*}
\frac{\tilde{C}_{\textrm{on}}}{\tilde{C}_{\textrm{off}}} &\leq \frac{\tilde{C}_{\textrm{on}}}{C_{\textrm{off}}}\\
& = \frac{\tilde{C}_{\textrm{on}}}{C_{\textrm{on}}}*\frac{C_{\textrm{on}}}{C_{\textrm{off}}}\\
&\leq \frac{\tilde{C}_{\textrm{on}}}{C_{\textrm{on}}}*\mathcal{CR}
\end{align*}
If $\frac{\tilde{C}_{\textrm{on}}}{C_{\textrm{on}}}\leq 1$, this theorem holds obviously; otherwise, we denote $\begin{cases}\tilde{C}_{\textrm{on}} = \tilde{C}_{\textrm{on}}^l+\tilde{C}_{\textrm{on}}^g\\ C_{\textrm{on}} = C_{\textrm{on}}^l+C_{\textrm{on}}^g\end{cases}$, where the superscripts $l$ and $g$ represent the costs from local generators and external grid respectively.
By Lemma~\ref{lemma:ramping_cost_grid}, we can have $\tilde{C}_{\textrm{on}}^g\leq C_{\textrm{on}}^g$; then
\begin{equation*}
\frac{\tilde{C}_{\textrm{on}}}{C_{\textrm{on}}}\leq \frac{\tilde{C}_{\textrm{on}}^n}{C_{\textrm{on}}^n}
\end{equation*}

Next we obtain an upper bound for $\frac{\tilde{C}_{\textrm{on}}^n}{C_{\textrm{on}}^n}$ by modifying the input a little bit. We expand each time slot to one segment by inserting $\frac{u(t)}{R}$ intervals with $0$ demand before $t$ and another $\frac{u(t)}{R}$ intervals with $0$ demands after $a(n)$.
Then, the online cost stays the same for the problem without ramping constraints. Furthermore, the online cost for the problem with ramping constraints increases.

For the $m^{th}$ segment,$C_{\textrm{on}}^n(m) = p_nu(m)$, while $\tilde{C}_{\textrm{on}}^n(m) =p_n( \sum_{i=1}^{\omega-1}iR+u(m)+\sum_{i=1}^{\omega-1}iR)\leq p_n*u(m)\omega$; meaning for any $m$ we can have
$$\frac{\tilde{C}_{\textrm{on}}^n(m)}{C_{\textrm{on}}^n(m)}\leq \omega$$

Then
\begin{align*}
\frac{\tilde{C}_{\textrm{on}}^n}{C_{\textrm{on}}^n} &=\frac{\sum_m\tilde{C}_{\textrm{on}}^n(m)}{\sum_mC_{\textrm{on}}^n(m)}\\
&\leq \omega
\end{align*}

Further we can have $\frac{\tilde{C}_{on}}{\tilde{C}_{off}}\leq \frac{C}{R}\mathcal{CR}$, which completes the proof.

\end{proof}
\fi 
